UniG3D: A Unified 3D Object Generation Dataset

The field of generative AI has a transformative impact on various areas, including virtual reality, autonomous driving, the metaverse, gaming, and robotics. Among these applications, 3D object generation techniques are of utmost importance. This technique has unlocked fresh avenues in the realm of creating, customizing, and exploring 3D objects. However, the quality and diversity of existing 3D object generation methods are constrained by the inadequacies of existing 3D object datasets, including issues related to text quality, the incompleteness of multi-modal data representation encompassing 2D rendered images and 3D assets, as well as the size of the dataset. In order to resolve these issues, we present UniG3D, a unified 3D object generation dataset constructed by employing a universal data transformation pipeline on Objaverse and ShapeNet datasets. This pipeline converts each raw 3D model into comprehensive multi-modal data representation <text, image, point cloud, mesh> by employing rendering engines and multi-modal models. These modules ensure the richness of textual information and the comprehensiveness of data representation. Remarkably, the universality of our pipeline refers to its ability to be applied to any 3D dataset, as it only requires raw 3D data. The selection of data sources for our dataset is based on their scale and quality. Subsequently, we assess the effectiveness of our dataset by employing Point-E and SDFusion, two widely recognized methods for object generation, tailored to the prevalent 3D representations of point clouds and signed distance functions. Our dataset is available at: https://unig3d.github.io.

==> Sections/7Supply.tex <==
\section{Experiments}

\subsection{Preliminary}
In this section, we provide a brief overview of two 3D object generation methods, Point-E and SDFusion, which are involved in the experimental part.

\subsubsection{Point-E}
Point-E builds upon the foundation established by previous research on diffusion-based models, which were first proposed by \cite{sohl2015deep} and popularized more recently~\cite{song2019generative, ho2020denoising}. It follows the Gaussian diffusion setup of \cite{ho2020denoising}. It aims to sample from some distribution $q(x_0)$ using a neural network approximation $p_\theta(x_0)$. Under Gaussian diffusion, it defines a noising process for integer timesteps $t \in [0,T]$.
%
\begin{equation}\label{noise_process}
q(x_t|x_{t-1}):=\mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1}, \beta_tI)
\end{equation}
%
Intuitively, this process gradually adds Gaussian noise to a signal over multiple timesteps. The magnitude of the noise added at each timestep is determined by a noise schedule, which is defined as $\beta_t$. Point-E employs a noise schedule such that, by the final timestep $t = T$, the sample $x_T$ contains almost no information. \cite{ho2020denoising}  note that it is possible to directly jump to a given timestep of the noising process without running the whole chain,
%
\begin{equation}\label{noise_chain}
x_t = \sqrt{\overline{\alpha}_t}x_0 + \sqrt{1-\overline{\alpha}_t}\epsilon
\end{equation}
%
where $\epsilon \sim \mathcal{N}(0, I)$ and $\overline{\alpha}_t := \prod_{s=0}^{t}1-\beta_t$. To train a diffusion model, Point-E approximate $q(x_t|x_{t-1})$ as a neural network $p_\theta(x_t|x_{t-1})$. It then produce a sample by starting at random Gaussian noise $x_T$ and gradually reversing the noising process until arriving at a noiseless sample $x_0$.
% \cite{karras2022elucidating} find that a carefully-designed second-order ODE solver provides a good trade-off between quality and sampling efficiency, and Point-E employ this sampler for its point cloud diffusion models. To trade off sample diversity for fidelity in diffusion models, Point-E utilizes classifier-free guidance, wherein a conditional diffusion model diffusion model $p(x_{t-1}|x_t, y)$ is trained with the class label stochastically dropped and replaced with an additional $\varnothing$ class. During sampling, the model’s output $\epsilon$ is linearly extrapolated away from the unconditional prediction towards the conditional prediction:
%
% \begin{equation}\label{epsilon_0}
% \epsilon_{guided} := \epsilon_{\theta}(x_t, \varnothing) + s \cdot (\epsilon_\theta(x_t, y)-\epsilon_\theta(x_t, \varnothing)
% \end{equation}
% %
% for some guidance scale $s \geq 1$. This approach is straightforward to implement, requiring only that conditioning information is randomly dropped during training time. Point-E employ this technique throughout its models, using the drop probability 0.1. 

% Rather than training a single generative model to directly produce point clouds conditioned on text, Point-E breaks the generation process into three steps. First, it generates a synthetic view conditioned on a text caption. Next, it produces a coarse point cloud (1,024 points) conditioned on the synthetic view. And finally, it produces a fine point cloud (4,096 points) conditioned on the low-resolution point cloud and the synthetic view. 
Due to training cost limitations, we only generate 1K coarse point clouds in our experiments. Additionally, we have not fine-tuned GLIDE on 3D renderings. Consequently, our experiments are conducted exclusively in text-conditioned.


\subsubsection{SDFusion}
% Given the computational complexity entailed, the direct application of diffusion models on reasonably high-resolution 3D shapes poses significant computational demands.
%
% SDFusion~\cite{cheng2022sdfusion}, a diffusion-based 3D generative model, solves this problem by using a signed distance function(SDF) as its 3D representation. 

Firstly, this method first compresses the 3D shape (SDF) into a discretized and compact latent space a latent space for diffusion through 3D-variant of the Vector Quantised-Variational AutoEncoder(VQ-VAE)~\cite{van2017neural}. Specifically, the employed 3D VQ-VAE contains an encoder $E_{\varphi}$ to encode the 3D shape into the latent space,
and a decoder $D_{\tau}$ to decode the latent vectors back to 3D space. 
% Given an input shape represented via the T-SDF X 
% $\in \mathbb{R}^{D\times{D}\times{D}}$, we have 
% \begin{equation}\label{epsilon_1}
% z=E_{\varphi}(X), \quad and \quad X'=D_{\tau}(VQ(z)), 
% \end{equation}
% where z $\in \mathbb{R}^{d\times{d}\times{d}}$is the latent vector, latent dimension $d$ is smaller than 3D shape dimension $D$, and VQ is the quantization step which maps the latent variable z to the nearest element in the codebook Z. The encoder $E_{\varphi}$, decoder $D_{\tau}$ , and codebook Z are jointly optimized. It pre-trains the VQ-VAE with reconstruction loss, commitment loss, and VQ objective.
%
Using the trained encoder $E_{\varphi}$, it can encode any given SDF into a compact and low-dimensional latent variable.  
Then, it trains a diffusion model on this latent representation. It uses the 3D diffusion model as an encoder-decoder to generate the latent space. Fundamentally, a diffusion model learns to sample from a target distribution by reversing a progressive noise diffusion process. Given a sample $z$, it obtains $z_t$,
$t \in \left\{ 1,\cdots, T\right\}$
by gradually adding Gaussian noise with a variance schedule. Then it uses a time-conditional 3D UNet 
$\epsilon_\theta$ 
as denoising model~\cite{ho2020denoising}. 
At inference time, it samples $z$ by gradually denoising a noise variable sampled from the standard normal distribution $N(0, 1)$, and leverages the trained VQ-VAE decoder $D_{\tau}$ to map the denoised code $\widehat{z}$ back to a 3D T-SDF shape representation.
This method further employ task-specific encoders followed by a cross-attention with various user conditions such as partial shapes, images, and text~\cite{rombach2022high}. 


\subsection{Hyperparameters of Model Training}
For the shape generation experiment utilizing SDFusion, we implement our networks using PyTorch and run all experiments on four GPU clusters with eight A100 GPUs. We train the generator, with the encoder, for 1,000,000 iterations with batch size 800 using the Adam optimizer with a learning rate of 1e-4. 

We train the point cloud diffusion model~\cite{nichol2022point} with batch size 64 for 50,000,000 iterations using the Adamw optimizer with a learning rate of 1e-5. In particular, we employ the 40M-text model structure in Point-E. The parameter number is around 40 million. Since Point-E does not provide the model training pipeline~\footnote{https://github.com/openai/point-e}, we reimplement it and release the code at: \href{https://github.com/Sense-GVT/unig3d_point-e
}{https://github.com/Sense-GVT/unig3d\_point-e.}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figures/wc_hd.jpg}
%     \vspace{-1em}
%     \caption{\Datasetname~Presentation. (a) Word cloud of text information. (b) Examples of multi-modal data representation in \Datasetname.
%     }
%     \label{fig:word_cloud}
%     % \vspace{-2em}
% \end{figure}

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-5em}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/wc_hd.jpg}
    % \vspace{-2em}
    \caption{Examples of multi-modal representation in \Datasetname.}
    \vspace{-2em}
    % \vspace{-0.5em}
\label{fig:word_cloud}
\end{wrapfigure}

\section{Showcase of \Datasetname}
% In this section, we provide an overview of our dataset by showcasing some examples. As shown in Fig.\ref{fig:word_cloud} (a), we present a word cloud of the textual information contained within the dataset. This visualization provides an at-a-glance summary of the most frequently occurring words in the text data.
%
% In addition to the word cloud, we also 
As shown in Fig.\ref{fig:word_cloud}, we demonstrate several examples of multi-modal data in quadruplet form. These examples showcase the different modalities of our dataset, including text, image, point cloud, and mesh. These quadruplets are representative of the overall dataset, which consists of millions of similar examples. 
%
Overall, these presentations provide a glimpse into the richness and diversity of our dataset, and demonstrate the potential for cross-modal applications. We encourage researchers from different domains to explore this dataset and use it for their own research purposes.

